GenAI Arena: An Open Evaluation Platform for Generative Models

Generative AI has made remarkable strides to revolutionize fields such as image and video generation. These advancements are driven by innovative algorithms, architecture, and data. However, the rapid proliferation of generative models has highlighted a critical gap: the absence of trustworthy evaluation metrics. Current automatic assessments such as FID, CLIP, FVD, etc often fail to capture the nuanced quality and user satisfaction associated with generative outputs. This paper proposes an open platform GenAI-Arena to evaluate different image and video generative models, where users can actively participate in evaluating these models. By leveraging collective user feedback and votes, GenAI-Arena aims to provide a more democratic and accurate measure of model performance. It covers three tasks of text-to-image generation, text-to-video generation, and image editing respectively. Currently, we cover a total of 35 open-source generative models. GenAI-Arena has been operating for seven months, amassing over 9000 votes from the community. We describe our platform, analyze the data, and explain the statistical methods for ranking the models. To further promote the research in building model-based evaluation metrics, we release a cleaned version of our preference data for the three tasks, namely GenAI-Bench. We prompt the existing multi-modal models like Gemini, and GPT-4o to mimic human voting. We compute the accuracy by comparing the model voting with the human voting to understand their judging abilities. Our results show existing multimodal models are still lagging in assessing the generated visual content, even the best model GPT-4o only achieves an average accuracy of 49.19 across the three generative tasks. Open-source MLLMs perform even worse due to the lack of instruction-following and reasoning ability in complex vision scenarios.

==> checklist.tex <==
\newpage
\section*{Checklist}

%%% BEGIN INSTRUCTIONS %%%
The checklist follows the references.  Please
read the checklist guidelines carefully for information on how to answer these
questions.  For each question, change the default \answerTODO{} to \answerYes{},
\answerNo{}, or \answerNA{}.  You are strongly encouraged to include a {\bf
justification to your answer}, either by referencing the appropriate section of
your paper or providing a brief inline description.  For example:
\begin{itemize}
  \item Did you include the license to the code and datasets? \answerYes{See Section~\ref{gen_inst}.}
  \item Did you include the license to the code and datasets? \answerNo{The code and the data are proprietary.}
  \item Did you include the license to the code and datasets? \answerNA{}
\end{itemize}
Please do not modify the questions and only use the provided macros for your
answers.  Note that the Checklist section does not count towards the page
limit.  In your paper, please delete this instructions block and only keep the
Checklist section heading above along with the questions/answers below.
%%% END INSTRUCTIONS %%%

\begin{enumerate}

\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{See section~\ref{intro}}
  \item Did you describe the limitations of your work?
    \answerYes{See section~\ref{sec:limit}}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerYes{See section~\ref{sec:impact}}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}

\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerNA{}
	\item Did you include complete proofs of all theoretical results?
    \answerNA{}
\end{enumerate}

\item If you ran experiments (e.g. for benchmarks)...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{See the \href{https://huggingface.co/spaces/TIGER-Lab/GenAI-Arena}{GenAI-Arena} demo URL on the first page.} 
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerNA{}
	\item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerYes{See appendix~\ref{appendix}}
	\item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{See section~\ref{sec:genai-museum}}
\end{enumerate}

\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{See section~\ref{sec:genai-museum}}
  \item Did you mention the license of the assets?
    \answerYes{See section~\ref{sec:genai_bench}}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerYes{See our released \href{https://huggingface.co/datasets/TIGER-Lab/GenAI-Bench}{GenAI-Bench}.}  
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerYes{See section~\ref{sec:data_collect}}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerYes{See section~\ref{sec:genai_bench}}
\end{enumerate}

\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerYes{Provided in the GenAI-Arena webpage.}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}

\end{enumerate}


==> correlation.tex <==
% % \begin{wraptable}{r}{0.7\textwidth}
% \begin{table}[h]
% \centering
% \caption{Correlation Study on existing metrics and human votings in GenAI-Bench.}
% \small
% \def\arraystretch{1.0}
% \setlength\tabcolsep{2 pt}
% \scalebox{0.9}{
% \begin{tabular}{lccc}
% \toprule
% \textbf{Metrics} & Text-To-Image & Image Editing & Text-To-Video \\
% \midrule
% Random                                         &  -0.0188    & -0.0293   & -0.0168   \\ 
% CLIPScore~\cite{hessel2021clipscore}           &  0.1450     & 0.1434    & 0.2643    \\ 
% %LPIPS~\cite{zhang2018perceptual}               &  N/A        & 0.2455    & N/A       \\ 
% GPT-4o~\cite{openai2023gpt4}-semantics         &  -0.0749    & -0.0314   & 0.0216        \\ 
% GPT-4o~\cite{openai2023gpt4}-quality           &  0.2259     & 0.0048    & 0.2169       \\ 
% GPT-4o~\cite{openai2023gpt4}-overall           &  -0.0233    & -0.0187   & 0.0393        \\ 
% Gemini-1.5-Pro~\cite{reid2024gemini}-semantics &  -0.0008    & 0.0997 & 0.0428\\ 
% Gemini-1.5-Pro~\cite{reid2024gemini}-visual    &  0.1725     & -0.0308 & -0.0388\\ 
% Gemini-1.5-Pro~\cite{reid2024gemini}-overall   &  0.0114     & 0.0916 & -0.0073\\ 
% Idefics2~\cite{laurençon2024matters}-semantics &  -0.0571    & 0.0325 & -0.1647\\ 
% Idefics2~\cite{laurençon2024matters}-visual    &  -0.1155     & -0.0363 & -0.0807\\ 
% Idefics2~\cite{laurençon2024matters}-overall   &  -0.0956     & 0.0101 & -0.1490\\ 
% %MiniCPM~\cite{hu2024minicpm}-semantics   &  TBA     & TBA & TBA\\ 
% %MiniCPM~\cite{hu2024minicpm}-visual   &  TBA     & TBA & TBA\\ 
% %MiniCPM~\cite{hu2024minicpm}-overall   &  TBA     & TBA & TBA\\ 
% Mantis~\cite{jiang2024mantis}-semantics   &  -0.0045     & -0.0754 & -0.0301\\ 
% Mantis~\cite{jiang2024mantis}-visual   &  0.0118     & -0.1006 & -0.0001\\ 
% Mantis~\cite{jiang2024mantis}-overall   &  -0.0078     & -0.1258 & 0.0050\\ 
% \bottomrule
% \end{tabular}}
% \label{tab:correlation}
% \end{table}
% % \end{wraptable}


\begin{table}[h]
\centering
\caption{Correlation Study on existing metrics and human votings in GenAI-Bench.}
\small
\def\arraystretch{1.0}
\setlength\tabcolsep{2 pt}
\begin{tabular}{l|ccc|ccc|ccc}
\toprule
Metrics        & \multicolumn{3}{c}{Text-To-Image} & \multicolumn{3}{c}{Image Editing} & \multicolumn{3}{c}{Text-To-Video} \\
\midrule
Subscore       & semantics   & quality  & overall  & semantics   & quality  & overall  & semantics   & quality  & overall  \\
\midrule
Random         & -0.0188     & -0.0188  & -0.0188  & -0.0293     & -0.0293  & -0.0293  & -0.0168     & -0.0168  & -0.0168  \\
CLIPScore~\cite{hessel2021clipscore}     & 0.1450      & 0.1450   & 0.1450   & 0.1434      & 0.1434   & 0.1434   & 0.2643      & 0.2643   & 0.2643   \\
GPT-4o~\cite{openai2023gpt4}         & -0.0749     & 0.2259   & -0.0233  & -0.0314     & 0.0048   & -0.0187  & 0.0216      & 0.2169   & 0.0393   \\
Gemini-1.5-Pro~\cite{reid2024gemini} & -0.0008     & 0.1725   & 0.0114   & 0.0997      & -0.0308  & 0.0916   & 0.0428      & -0.0388  & -0.0073  \\
Idefics2~\cite{laurençon2024matters}       & -0.0571     & -0.1155  & -0.0956  & 0.0325      & -0.0363  & 0.0101   & -0.1647     & -0.0807  & -0.1490  \\
Mantis~\cite{jiang2024mantis}         & -0.0045     & 0.0118   & -0.0078  & -0.0754     & -0.1006  & -0.1258  & -0.0301     & -0.0001  & 0.0050   \\
\bottomrule
\end{tabular}
\label{tab:correlation}
\end{table}

==> full_leaderboard.tex <==
\begin{table}[!t]
    \small
    \centering
    \vspace{-2em}
    \caption{GenAI-Arena Leaderboards. \\(Last updated on Oct 24th, 2024)}
    \scalebox{0.99}{
    \begin{minipage}[b]{0.32\textwidth}
        \centering
        \subcaption{Text-to-Image}
        \scalebox{0.85}{
        \begin{tabular}{lcc}
            \toprule
            Model & Elo & 95\% CI \\
            \midrule
            PlayGround V2.5 & 1122 & +19/-20 \\
            FLUX.1-dev    & 1114 & +45/-42 \\
            FLUX.1-schnell & 1085 & +43/-46 \\
            Playground V2 & 1072 & +18/-22 \\
            Kolors & 1069 & +32/-39 \\
            StableCascade & 1057 & +17/-21 \\
            HunyuanDiT & 1030 & +25/-27 \\
            PixArt-$\alpha$ & 1020 & +17/-19 \\
            SDXL-Lightning & 1020 & +17/-15 \\
            PixArt-$\sigma$ & 1019 & +22/-20 \\
            SD3 & 1007 & +37/-33 \\
            AuraFlow & 1003 & +45/-58 \\
            SDXL & 965 & +14/-15 \\
            SDXL-Turbo & 913 & +14/-14 \\
            LCM & 905 & +26/-26 \\
            OpenJourney & 828 & +17/-15 \\
            \bottomrule
        \end{tabular}}
        \label{tab:t2i_ranking}
    \end{minipage}
    \hfill
    \begin{minipage}[b]{0.30\textwidth}
        \centering
        \subcaption{Image Editing}
        \scalebox{0.85}{
        \begin{tabular}{lcc}
            \toprule
            Model & Elo & 95\% CI \\
            \midrule
            MagicBrush & 1108 & +32/-28 \\
            InfEdit & 1075 & +26/-32 \\
            CosXLEdit & 1066 & +31/-29 \\
            InstructPix2Pix & 1038 & +32/-24 \\
            PNP & 998 & +35/-34 \\
            Prompt2prompt & 988 & +26/-23 \\
            CycleDiffusion & 943 & +26/-26 \\
            SDEdit & 924 & +24/-23 \\
            Pix2PixZero & 858 & +25/-30 \\
            \\
            \\
            \\
            \\
            \\
            \\
            %LEDITS      &     &         &     \\
            \bottomrule
        \end{tabular}}
        \label{tab:i2i_ranking}
    \end{minipage}
    \hfill
    \begin{minipage}[b]{0.33\textwidth}
        \centering
        \subcaption{Text-to-Video}
        \scalebox{0.85}{
        \begin{tabular}{lcc}
        \toprule
        Model & Elo & 95\% CI \\
        \midrule
        StableVideoDiffusion & 1148 & +31/-28 \\
        CogVideoX-2B & 1106 & +71/-71 \\
        T2V-Turbo & 1085 & +36/-32 \\
        VideoCrafter2 & 1068 & +20/-22\\
        AnimateDiff & 1068 & +25/-21 \\
        LaVie & 996 & +25/-21 \\
        OpenSora & 912 & +23/-23 \\
        OpenSora v1.2 & 894 & +54/-71 \\
        ModelScope & 862 & +25/-22 \\
        AnimateDiff-Turbo & 861 & +22/-20 \\
        \\
        \\
        \\
        \\
        \\
        \bottomrule
        \end{tabular}}
        \label{tab:t2v_ranking}
    \end{minipage}}
    \hfill
    \label{tab:leaderboard}
\end{table}


==> genai_bench_pairwise_acc_poster.tex <==

\begin{table}[h]
\centering
\small
\def\arraystretch{1.0}
\setlength\tabcolsep{2 pt}
\begin{tabular}{lcccc}
\toprule
Model                    & Image Generation & Image Editing & Video Generation & Average \\
\midrule
Random                   & 25.36\%          & 25.90\%       & 25.16\%          & 25.47\% \\
\midrule
Idefics1                 & 0.81\%           & 5.66\%        & 0.19\%           & 2.22\%  \\
InstructBLIP             & 3.11\%           & 19.80\%       & 3.74\%           & 8.89\%  \\
QwenVL                   & 26.63\%          & 14.91\%       & 2.15\%           & 14.56\% \\
CogVLM                   & 29.34\%          & 0.00\%        & 24.60\%          & 17.98\% \\
VideoLLaVA               & 37.75\%          & 26.66\%       & 0.00\%           & 21.47\% \\
BLIP-2                   & 26.34\%          & 26.01\%       & 16.93\%          & 23.09\% \\
MiniCPM-V-2.5            & 37.81\%          & 25.24\%       & 6.55\%           & 23.20\% \\
LLaVA-1.6-7B             & 22.65\%          & 25.35\%       & 21.70\%          & 23.24\% \\
Idefics2                 & 42.25\%          & 27.31\%       & 16.46\%          & 28.67\% \\
LLaVA-1.5-7B             & 37.00\%          & 26.12\%       & 30.40\%          & 31.17\% \\
Gemini-1.5-Pro           & 44.67\%          & \textbf{55.93}\% & 46.21\%       & 48.94\% \\
GPT-4o                   & \textbf{45.59}\% & 53.54\%       & \textbf{48.46}\% & \textbf{49.19}\% \\
\bottomrule
\end{tabular}
\end{table}


==> leaderboard-t2v.tex <==
\begin{table}[!h]
    \small
    \centering
    \scalebox{0.99}{
    \begin{minipage}[b]{0.5\textwidth}
        \centering
        \scalebox{1}{
        \begin{tabular}{lccc}
            \toprule
            Model & Elo & 95\% CI & Votes \\
            \midrule
            PlayGround V2.5 & 1150 & +21/-22 & 524 \\
            Playground V2 & 1101 & +14/-20 & 1042 \\
            StableCascade & 1057 & +20/-24 & 634 \\
            SDXLLightning & 1053 & +22/-22 & 605 \\
            PixArtAlpha & 1052 & +15/-19 & 1098 \\
            PixArtSigma & 1050 & +26/-23 & 428 \\
            SDXL & 1001 & +15/-14 & 1112 \\
            SDXLTurbo & 935 & +18/-16 & 1158 \\
            OpenJourney & 853 & +13/-17 & 1140 \\
            LCM & 817 & +20/-20 & 736 \\
            \bottomrule
        \end{tabular}}
        \caption{Text-to-Image.}
        \label{tab:t2i_ranking}
    \end{minipage}
    \hfill
    \begin{minipage}[b]{0.32\textwidth}
        \centering
        \scalebox{1}{
        \begin{tabular}{lccc}
            \toprule
            Model & Elo & 95\% CI & Votes \\
            \midrule
            MagicBrush & 1111 & +28/-32 & 277 \\
            InFEdit & 1079 & +27/-33 & 223 \\
            CosXLEdit & 1066 & +31/-30 & 228 \\
            InstructPix2Pix & 1033 & +32/-26 & 235 \\
            PNP & 998 & +37/-36 & 236 \\
            Prompt2prompt & 988 & +25/-25 & 252 \\
            CycleDiffusion & 939 & +23/-26 & 230 \\
            SDEdit & 929 & +25/-21 & 237 \\
            Pix2PixZero & 857 & +20/-24 & 248 \\
            %LEDITS      &     &         &     \\
            \bottomrule
        \end{tabular}}
        \caption{Image editing.}
        \label{tab:i2i_ranking}
    \end{minipage}
    \hfill
    \begin{minipage}[b]{0.5\textwidth}
        \centering
        \scalebox{1}{
        \begin{tabular}{lccc}
        \toprule
        Model & Elo & 95\% CI & Votes \\
        \midrule
        T2VTurbo & 1113 & +53/-46 & 131 \\
        StableVDiffusion & 1105 & +45/-37 & 192 \\
        VideoCrafter2 & 1077 & +18/-18 & 468 \\
        AnimateDiff & 1075 & +23/-26 & 455 \\
        LaVie & 997 & +24/-26 & 462 \\
        OpenSora & 916 & +19/-23 & 477 \\
        ModelScope & 866 & +19/-22 & 437 \\
        AnimateDiffTurbo & 851 & +18/-20 & 514 \\
        \bottomrule
        \end{tabular}}
        \caption{Text-to-video.}
        \label{tab:t2v_ranking}
    \end{minipage}}
    \caption{Arena Leaderboard Results.}
\end{table}


==> leaderboard_poster.tex <==
\begin{table}[!t]
    \small
    \centering
    \vspace{-2em}
    \scalebox{0.99}{
    \begin{minipage}[b]{0.30\textwidth}
        \centering
        \subcaption*{Text-to-Image}
        \scalebox{0.85}{
        \begin{tabular}{lcc}
            \toprule
            Model & Elo & Votes \\
            \midrule
            PlayGround V2.5 & 1122 & 926 \\
            FLUX.1-dev & 1114 & 141 \\
            FLUX.1-schnell & 1085 & 171 \\
            PlayGround V2 & 1072 & 1050 \\
            Kolors & 1069 & 153 \\
            StableCascade & 1039 & 953 \\
            HunyuanDiT & 1030 & 291 \\
            PixArtAlpha & 1020 & 1405 \\
            SDXL-Lightning & 1020 & 921 \\

            \bottomrule
        \end{tabular}}
    \end{minipage}
    \hfill
    \begin{minipage}[b]{0.28\textwidth}
        \centering
        \subcaption*{Image Editing}
        \scalebox{0.85}{
        \begin{tabular}{lcc}
            \toprule
            Model & Elo & Votes \\
            \midrule
            MagicBrush & 1108 & 292 \\
            InfEdit & 1075 & 240 \\
            CosXLEdit & 1066 & 241 \\
            InstructPix2Pix & 1038 & 257 \\
            PNP & 998 & 255 \\
            Prompt2prompt & 988 & 266 \\
            CycleDiffusion & 943 & 244 \\
            SDEdit & 924 & 253 \\
            Pix2PixZero & 858 & 260 \\

            %LEDITS      &     &         &     \\
            \bottomrule
        \end{tabular}}
    \end{minipage}
    \hfill
    \begin{minipage}[b]{0.30\textwidth}
        \centering
        \subcaption*{Text-to-Video}
        \scalebox{0.85}{
        \begin{tabular}{lcc}
        \toprule
        Model & Elo & Votes \\
        \midrule
        StableVDiffusion & 1148 & 343 \\
        CogVideoX-2B & 1106 & 66\\
        T2V-Turbo & 1075 & 232 \\
        VideoCrafter2 & 1068 & 574 \\
        AnimateDiff & 1068 & 573 \\
        LaVie & 996 & 518 \\
        OpenSora & 912 & 527 \\
        OpenSora v1.2 & 894 & 79 \\
        ModelScope & 862 & 495 \\

        \bottomrule
        \end{tabular}}
    \end{minipage}}
    \hfill
\end{table}

